How to Synthesize Text Data without Model Collapse?

Model collapse in synthetic data indicates that iterative training on self-generated data leads to a gradual decline in performance. With the proliferation of AI models, synthetic data will fundamentally reshape the web data ecosystem. Future GPT-$\{n\}$ models will inevitably be trained on a blend of synthetic and human-produced data. In this paper, we focus on two questions: what is the impact of synthetic data on language model training, and how to synthesize data without model collapse? We first pre-train language models across different proportions of synthetic data, revealing a negative correlation between the proportion of synthetic data and model performance. We further conduct statistical analysis on synthetic data to uncover distributional shift phenomenon and over-concentration of n-gram features. Inspired by the above findings, we propose token editing on human-produced data to obtain semi-synthetic data. As a proof of concept, we theoretically demonstrate that token-level editing can prevent model collapse, as the test error is constrained by a finite upper bound. We conduct extensive experiments on pre-training from scratch, continual pre-training, and supervised fine-tuning. The results validate our theoretical proof that token-level editing improves model performance.

==> useless_figures.tex <==

% \begin{figure}[th!]
%     % \vspace{-2em}
%     \centering
%     \begin{center}
%         \includegraphics[width=\linewidth]{figures/token_probs.pdf}
%         % \vspace{-2em}
%         \caption{U-shape token probability distribution of Dolma-sampled V6 estimated by Qwen-0.5B-Instruct~\citep{qwen2}.}
%         \label{fig:qwen2_probs}
%     \end{center}
%     % \vspace{-2em}
% \end{figure}

\begin{figure*}[t]
% \vspace{-4em}
  \centering
  \includegraphics[width=\linewidth]{figures/tsne_and_dsir_ppl.pdf}
  \vspace{-2em}
  \caption{\textbf{A.} Embedding visualization using t-SNE and sentence-transformers. \textbf{B.} pre-training results for selected synthetic data and other data mixtures.} 
  \label{fig:tsne_and_dsir_ppl}
  \vspace{-1em}
\end{figure*}

\begin{figure*}[t!]
% \vspace{-4em}
\small
  \centering
  \includegraphics[width=\linewidth]{figures/non-iterative_model_collapse.pdf}
  \vspace{-2em}
  \caption{Non-iterative model collapse. Training language models from scratch on AI-synthesized data or a mixture of human and synthetic data leads to performance degradation. This degradation is negatively correlated with the proportion of synthetic data used in training. 
  \textbf{A.} We pre-train GPT-2 Small (124M) on human (Dolma~\citep{dolma}) and synthetic (Cosmopedia~\citep{benallal2024cosmopedia}) data. As the proportion of synthetic data increases, the model’s loss decreases. \textbf{B.} 
  As the proportion of synthetic data increases, the PPL also rises. This trend remains consistent across different validation sets. More results on downstream tasks are presented in~\ref{tab:human_vs_synthetic_downstream_tasks} and ~\ref{tab:human_vs_synthetic_downstream_tasks_olmo}. 
  % and~\ref{tab:ppl_results_of_pile}.
  } 
  \label{fig:gpt2-pretraining-and-eval}
  % \vspace{-1em}
\end{figure*}

\begin{table*}[t]
\centering
\caption{Subdomain PPL evaluation results for GPT-2 Small (124M) pre-trained on data mixture. The PPL increases as the proportion of synthetic data grows, providing further confirmation of Figure~\ref{fig:gpt2-pretraining-and-eval}.}
\label{tab:ppl_results_of_pile}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccccccccc|c}
        \toprule
        \textbf{} & \textbf{ArXiv} & \textbf{Books2} & \textbf{Books3} & \textbf{Math} & \textbf{Enron} & \textbf{EuroParl} & \textbf{FreeLaw} & \textbf{GitHub} & \textbf{PG-19} & \textbf{HackerNews} & \textbf{NIH} \\ 
        \midrule
        Human data         & \colorone{22.26} & \colorone{25.39} & \colorone{22.87} & \colorone{10.84} & \colorone{23.50} & \colorone{30.73} & \colorone{12.04} & \colorone{4.15} & \colorone{16.88} & \colorone{32.54} & \colorone{23.53} \\ 
        25\% Synthetic Data & \colorone{21.86} & \colorone{26.32} & \colortwo{23.87} & \colorone{11.05} & \colortwo{24.85} & \colortwo{35.02} & \colortwo{12.84} & \colortwo{4.35} & \colortwo{17.99} & \colortwo{33.80} & \colortwo{23.76} \\ 
        50\% Synthetic Data & \colortwo{22.50} & \colortwo{28.01} & \colorthree{25.75} & \colorone{10.84} & \colorthree{26.56} & \colorthree{41.99} & \colorthree{14.02} & \colorthree{4.67} & \colorthree{19.70} & \colorthree{36.12} & \colorthree{24.61} \\ 
        75\% Synthetic Data & \colorthree{24.35} & \colorthree{31.19} & \colorfour{28.98} & \colortwo{11.81} & \colorfour{30.30} & \colorfour{56.32} & \colorfour{16.03} & \colorfour{5.30} & \colorfour{22.75} & \colorfour{40.44} & \colorfour{26.19} \\ 
        Synthetic Data     & \colorfive{35.60} & \colorfive{43.72} & \colorfive{47.72} & \colorfive{17.25} & \colorfive{66.97} & \colorfive{129.75} & \colorfive{29.62} & \colorfive{12.00} & \colorfive{50.14} & \colorfive{87.95} & \colorfive{39.48} \\ 
        \midrule
        \midrule
        \textbf{} & \textbf{OpenSubts} & \textbf{OWT2} & \textbf{Phil} & \textbf{Pile-CC} & \textbf{PubMed-A} & \textbf{PubMed-C} & \textbf{StackEx} & \textbf{Ubuntu} & \textbf{USPTO} & \textbf{Wikipedia} & \textbf{Youtube} & \textbf{Avg} \\ 
        \midrule
        Human data & \colorone{28.08} & \colorone{25.77} & \colorone{33.56} & \colorone{26.78} & \colorone{18.97} & \colorone{15.49} & \colorone{10.81} & \colorone{20.86} & \colorone{19.32} & \colorone{24.31} & \colorone{21.54} & \colorone{21.37} \\ 
        25\% Synthetic Data & \colortwo{29.25} & \colortwo{26.94} & \colortwo{34.63} & \colortwo{27.83} & \colortwo{19.55} & \colortwo{15.38} & \colortwo{11.03} & \colortwo{22.32} & \colortwo{19.58} & \colortwo{25.88} & \colortwo{22.63} & \colortwo{22.31} \\ 
        50\% Synthetic Data & \colorthree{31.00} & \colorthree{28.76} & \colorthree{37.48} & \colorthree{29.36} & \colorthree{20.51} & \colorthree{15.89} & \colorthree{11.54} & \colorthree{23.53} & \colorthree{20.51} & \colorthree{27.57} & \colorthree{24.91} & \colorthree{23.90} \\ 
        75\% Synthetic Data & \colorfour{34.18} & \colorfour{32.04} & \colorfour{42.39} & \colorfour{32.17} & \colorfour{22.33} & \colorfour{16.92} & \colorfour{12.55} & \colorfour{26.54} & \colorfour{22.21} & \colorfour{30.68} & \colorfour{28.98} & \colorfour{27.03} \\ 
        Synthetic Data     & \colorfive{57.83} & \colorfive{53.94} & \colorfive{78.18} & \colorfive{54.69} & \colorfive{34.82} & \colorfive{23.87} & \colorfive{20.47} & \colorfive{51.78} & \colorfive{37.24} & \colorfive{46.12} & \colorfive{65.49} & \colorfive{49.30} \\ 
        \bottomrule
    \end{tabular}} 
\end{table*}
